Dark matter scattering off ${}^4$He in chiral effective field theory

We study dark matter scattering off ${}^4$He and other light nuclei using chiral effective field theory. We consider scalar DM interactions and include both one- and two-nucleon scattering processes. The DM interactions and nuclear wave functions are obtained from chiral effective field theory and we work up to fourth order in the chiral expansion for the latter to investigate the chiral convergence. The results for the scattering rates can be used to determine the sensitivity of planned experiments to detect relatively light dark matter particles using ${}^4$He. We find that next-to-leading-order scalar currents are smaller than expected from power counting for scattering off ${}^4$He confirming earlier work. However, the results for two-nucleon corrections exhibit a linear regulator dependence indicating potential problems in the applied power counting. We observe a linear correlation between the, in principle not observable, D-wave probability of various light nuclei and the scalar two-nucleon matrix elements, again pointing towards potentially missing contributions.

==> Appx_operators.tex <==
\red{I copied from the paper, are we including this?}

The computation of the spin-independent scattering matrix in Eq. (\ref{eq:mel_jmj}) involves the sum (average) over all outgoing (incoming) nuclear polarizations.  This summation can be simplified in terms of reduced matrix elements
\begin{equation}
	\braket{ j' m_j' | \hat{\mathcal{O}} _ {\xi m_\xi} | j m_j  }
	=
	\CG{j}{\xi}{j'}{m_j}{m_\xi}{m_j'}
	\braket{j' | \hat{\mathcal{O}} _ {\xi} | j}
	\ .
\end{equation}
Eq. (\ref{eq:mel_jmj}) then becomes
\begin{equation}
	\abs{ \mathcal{M}_A ( \vec q ^2) }^2 = 
	(2 m_T )^2( 2 m_\chi )^2
	\sum_{\xi=0}^\infty
	\abs{
		\Braket{ \Psi_T, j | \ \hat{ J } (\vec q ^2, \xi) \ | \Psi_T, j }
	}^2 \ .
\end{equation}
In the limit of $q \rightarrow 0$, one can show that for spin-conserving structures, only contributions with $\xi=0$ survive.  Following Eq. (\ref{eq:Fi_def}), we further define
\begin{equation}
	\label{def:op_expectation_value}
	\braket{ \hat J_a }_T
	:=
	\frac{
		\Braket{ \Psi_T, j | \ \hat{ J }_{ a} (\vec q ^2, \xi) \ | \Psi_T, j }
	}{A \, \abs{ \sigma_{\pi N} \ c_{\chi} } } \Bigg|_{\xi=0}
	\ .
\end{equation}
For benchmarking purposes, we present the expectation values for the isoscalar quark-DM two-nucleon contributions at $\vec q=0$  in Table \ref{tab:amp_res}.  We estimate the numerical uncertainty to be below the  $1 \%$-level with respect to the value of each matrix element.

%\comment{*Concerning Table V}{Andreas}{need to convert to e.g. $ -9.78 \cdot 10^{-4}$} 

\begin{table}
\scriptsize
\centering
\begin{tabular}{l | rrr}
NN interaction &     $\braket{ \hat J_{q^{(\mathrm{is})},2b} }_{^2\mathrm{H}}$ &     $\braket{\hat J_{q^{(\mathrm{is})},2b} }_{^3\mathrm{H}}$ &    $\braket{\hat J_{q^{(\mathrm{is})},2b} }_{^3\mathrm{He}}$ \\[0.4em]
\hline\hline
AV18 + Urb IXF          &         / &  2.62$\cdot 10^{-3}$ &  2.52$\cdot 10^{-3}$ \\[-0.4em]
AV18                    &  1.58$\cdot 10^{-4}$ &  2.62$\cdot 10^{-3}$ &  2.83$\cdot 10^{-3}$ \\[-0.4em]
CD-Bonn + TM            &         / &  1.38$\cdot 10^{-3}$ &  1.51$\cdot 10^{-3}$ \\[-0.4em]
CD-Bonn                 &  1.17$\cdot 10^{-4}$ &  1.47$\cdot 10^{-3}$ &  1.62$\cdot 10^{-3}$ \\[-0.4em]
NIJM                    &  1.57$\cdot 10^{-4}$ &         / &         / \\
\hline
LO\,\,\,\,\,\, $(Q^0)$   $\Lambda_{1}$ &  2.28$\cdot 10^{-3}$ & -1.46$\cdot 10^{-3}$ & -1.45$\cdot 10^{-3}$ \\[-0.4em]
LO\,\,\,\,\,\, $(Q^0)$   $\Lambda_{2}$ & -5.95$\cdot 10^{-4}$ & -1.77$\cdot 10^{-3}$ & -1.77$\cdot 10^{-3}$ \\[-0.4em]
LO\,\,\,\,\,\, $(Q^0)$   $\Lambda_{3}$ & -2.66$\cdot 10^{-3}$ & -2.01$\cdot 10^{-3}$ & -2.02$\cdot 10^{-3}$ \\[-0.4em]
LO\,\,\,\,\,\, $(Q^0)$   $\Lambda_{4}$ & -4.12$\cdot 10^{-3}$ & -2.20$\cdot 10^{-3}$ & -2.22$\cdot 10^{-3}$ \\[-0.4em]
LO\,\,\,\,\,\, $(Q^0)$   $\Lambda_{5}$ & -5.13$\cdot 10^{-3}$ & -2.36$\cdot 10^{-3}$ & -2.38$\cdot 10^{-3}$ \\
\hline 
NLO\,\, ($Q^{2}$)    $\Lambda_{1}$ &  1.17$\cdot 10^{-4}$ &  1.48$\cdot 10^{-3}$ &  1.62$\cdot 10^{-3}$ \\[-0.4em]
NLO\,\, ($Q^{2}$)    $\Lambda_{2}$ &  8.80$\cdot 10^{-3}$ &  7.08$\cdot 10^{-4}$ &  8.18$\cdot 10^{-4}$ \\[-0.4em]
NLO\,\, ($Q^{2}$)    $\Lambda_{3}$ &  6.09$\cdot 10^{-3}$ &  2.72$\cdot 10^{-5}$ &  1.08$\cdot 10^{-4}$ \\[-0.4em]
NLO\,\, ($Q^{2}$)    $\Lambda_{4}$ &  3.70$\cdot 10^{-3}$ & -5.47$\cdot 10^{-4}$ & -4.91$\cdot 10^{-4}$ \\[-0.4em]
NLO\,\, ($Q^{2}$)    $\Lambda_{5}$ &  1.65$\cdot 10^{-3}$ & -1.01$\cdot 10^{-3}$ & -9.78$\cdot 10^{-4}$ \\
\hline 
N${}^2$LO ($Q^{3}$)   $\Lambda_{1}$ &  1.10$\cdot 10^{-4}$ &  1.37$\cdot 10^{-3}$ &  1.51$\cdot 10^{-3}$ \\[-0.4em]
N${}^2$LO ($Q^{3}$)   $\Lambda_{2}$ &  8.59$\cdot 10^{-3}$ &  7.25$\cdot 10^{-4}$ &  8.39$\cdot 10^{-4}$ \\[-0.4em]
N${}^2$LO ($Q^{3}$)   $\Lambda_{3}$ &  6.17$\cdot 10^{-3}$ &  1.06$\cdot 10^{-4}$ &  1.93$\cdot 10^{-4}$ \\[-0.4em]
N${}^2$LO ($Q^{3}$)   $\Lambda_{4}$ &  3.97$\cdot 10^{-3}$ & -4.39$\cdot 10^{-4}$ & -3.75$\cdot 10^{-4}$ \\[-0.4em]
N${}^2$LO ($Q^{3}$)   $\Lambda_{5}$ &  2.04$\cdot 10^{-3}$ & -8.98$\cdot 10^{-4}$ & -8.55$\cdot 10^{-4}$ \\
\hline 
N${}^3$LO ($Q^{4}$)   $\Lambda_{1}$ &  7.31$\cdot 10^{-3}$ &  7.54$\cdot 10^{-4}$ &  8.61$\cdot 10^{-4}$ \\[-0.4em]
N${}^3$LO ($Q^{4}$)   $\Lambda_{2}$ &  1.09$\cdot 10^{-4}$ &  1.66$\cdot 10^{-3}$ &  1.81$\cdot 10^{-3}$ \\[-0.4em]
N${}^3$LO ($Q^{4}$)   $\Lambda_{3}$ &  1.29$\cdot 10^{-4}$ &  2.21$\cdot 10^{-3}$ &  2.38$\cdot 10^{-3}$ \\[-0.4em]
N${}^3$LO ($Q^{4}$)   $\Lambda_{4}$ &  1.37$\cdot 10^{-4}$ &  2.44$\cdot 10^{-3}$ &  2.62$\cdot 10^{-3}$ \\[-0.4em]
N${}^3$LO ($Q^{4}$)   $\Lambda_{5}$ &  1.38$\cdot 10^{-4}$ &  2.50$\cdot 10^{-3}$ &  2.69$\cdot 10^{-3}$ \\
\hline 
N${}^4$LO ($Q^{5}$)   $\Lambda_{1}$ &  1.06$\cdot 10^{-4}$ &  1.62$\cdot 10^{-3}$ &  1.77$\cdot 10^{-3}$ \\[-0.4em]
N${}^4$LO ($Q^{5}$)   $\Lambda_{2}$ &  1.13$\cdot 10^{-4}$ &  1.77$\cdot 10^{-3}$ &  1.92$\cdot 10^{-3}$ \\[-0.4em]
N${}^4$LO ($Q^{5}$)   $\Lambda_{3}$ &  1.18$\cdot 10^{-4}$ &  1.91$\cdot 10^{-3}$ &  2.07$\cdot 10^{-3}$ \\[-0.4em]
N${}^4$LO ($Q^{5}$)   $\Lambda_{4}$ &  1.25$\cdot 10^{-4}$ &  2.10$\cdot 10^{-3}$ &  2.27$\cdot 10^{-3}$ \\[-0.4em]
N${}^4$LO ($Q^{5}$)   $\Lambda_{5}$ &  1.27$\cdot 10^{-4}$ &  2.20$\cdot 10^{-3}$ &  2.38$\cdot 10^{-3}$ \\
\end{tabular}
\caption{\label{tab:amp_res}%
Central values for spin-independent isoscalar-quark two-pion-exchange operators $\hat J_{q^{(\mathrm{is})},2b}$ for all applied wave functions at zero momentum transfer $\vec q=0$. Fore more details, we refer to Appendix \ref{Appx_operators}.%
}
\end{table}


